A generalized Gross-Pitaevskii model for intersubband polariton lasing

We develop a generalized Gross-Pitaevskii approach to the driven-dissipative dynamics of intersubband polaritons in patterned planar microcavities where the cavity mode is strongly coupled to an intersubband transition in doped quantum wells. Substantial differences with respect to the case of interband excitonic polaritons are highlighted, in particular the non-Markovian features of the radiative decay. The accuracy of the method is validated on the linear reflection properties of the cavity, that quantitatively reproduce experimental observations. The theoretical framework is then applied in the nonlinear regime to study optical parametric oscillation processes for intersubband polaritons. Our findings open interesting perspectives in view of novel coherent laser sources operating in the mid and far infrared.

==> img/nonmarkov.tex <==
\begin{tikzpicture}
 \draw [->] (-3, 0) -- (3.5, 0) node[anchor=west] {$k$};
 \draw [->] (0, -0.1) -- (0, 3) node[anchor=west] {$\omega$};
 
 % lightcone
 \draw [black, very thick] (0, 0) -- ( 2.5, 2.5) node[anchor=west] {LC};
 \draw [black, very thick] (0, 0) -- (-2.5, 2.5);
 
 % cavity
 \draw [black, thick, dashed] (0, 0) -- ( 3.3, 1.65) node[anchor=west] 
{$\omega_C(k)$};
 \draw [black, thick, dashed] (0, 0) -- (-2.8, 1.4);
 
 % hops
 \draw [->]         (0.5,1.5) arc (180:0:0.6) node[midway, above] {$k_B$};
 \draw [->]         (1.7,1.5) arc (180:0:0.6) node[midway, above] {};
 \draw [->, dashed] (2.9,1.5) arc (180:100:0.6);
 
 \draw [->]         ( 0.5,1.5) arc (0:180:0.6) node[midway, above] {$k_B$};
 \draw [->]         (-0.7,1.5) arc (0:180:0.6) node[midway, above] {$k_B$};
 \draw [->, dashed] (-1.9,1.5) arc (0:120:0.6);
 
 \fill ( 0.5,1.5) circle (0.1);
 \draw [very thick] ( 2.9,1.5) circle (0.1);
 \draw [densely dotted] (0.5, 1.5) -- (0.5, 0) node[anchor=north]{$k_p$};
 \draw [densely dotted] (0.5, 1.5) -- (0, 1.5) node[anchor=east] {$\omega_p$};
\end{tikzpicture}


